Trust but Verify! A Survey on Verification Design for Test-time Scaling

Test-time scaling (TTS) has emerged as a new frontier for scaling the performance of Large Language Models. In test-time scaling, by using more computational resources during inference, LLMs can improve their reasoning process and task performance. Several approaches have emerged for TTS such as distilling reasoning traces from another model or exploring the vast decoding search space by employing a verifier. The verifiers serve as reward models that help score the candidate outputs from the decoding process to diligently explore the vast solution space and select the best outcome. This paradigm commonly termed has emerged as a superior approach owing to parameter free scaling at inference time and high performance gains. The verifiers could be prompt-based, fine-tuned as a discriminative or generative model to verify process paths, outcomes or both. Despite their widespread adoption, there is no detailed collection, clear categorization and discussion of diverse verification approaches and their training mechanisms. In this survey, we cover the diverse approaches in the literature and present a unified view of verifier training, types and their utility in test-time scaling. Our repository can be found at https://github.com/elixir-research-group/Verifierstesttimescaling.github.io.

==> 03-framework-AA.tex <==
%\input{tables/taxonomy}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/taxonomy_verifiers-cropped.pdf}
%     \caption{A taxonomy of verification approaches aiding in test-time scaling}
%     \label{fig:enter-label}
% \end{figure}
\input{figures/taxonomy-forest}


\begin{figure*}
    \centering
    \includegraphics[width=0.88\linewidth]{figures/verifier-suervey-cropped.pdf}
    \caption{An overview of  verifier training mechanisms}
    \label{fig:unified_framework}
\end{figure*}
 \section{Approaches for Verifier Training and Verifier Types}
 \label{sec:methods}


The verifiers are categorized based on their usage and what aspect they verify, as discussed in the previous section. They could further be analyzed based on their training objectives, type of training data generation or based on the type of function employed as verifier.
 
 In this section, we cover diverse aspects of verifier training approaches and discuss the advantages and limitations of the specific approaches based on use cases. Figure \ref{fig:unified_framework} present a generalized view of different mechanisms for training or employing verifiers for TTS encompassing the data generation (synthetic reasoning steps vs human annotated), annotation mechanisms (automated step-level or outcome-level scores vs manual), verifier types (neuro-symbolic, tool-based, LLM-based, LRM-based) and training objectives namely supervised fine-tuning (SFT) or RL-based. An overview of our fine-grained taxonomy for categorizing verifiers is shown in Figure \ref{fig:categorization_tree}.
 % \vspace{-0.9em}

 \subsection{Heuristic verifiers} 
Early verification strategies primarily relied on heuristics to verify final solutions such as output fluency, plausibility, adherence to format \cite{deepseek-r1} where LLMs are trained to self-verify using these heuristics as rewards for RL-based training using Group Relative Policy Optimization (GRPO). RvLLM \cite{rvllm_rule_based} designs an Expert Specification language (ESL) that can be used by experts to design domain specific rules for verification. However, rule based verification approaches are not scalable as it is time-consuming to author comprehensive rules. They may also fail to capture semantic variations in expression (for example: ``2 hours" and ``120 minutes" imply the same) resulting in incorrect verification. Hence, model-based verifiers are proposed as covered in subsequent sections.                    

\subsection{Discriminative verifiers}

LLM-based verifiers are usually trained as discriminative models that can assign scores to candidate solution paths to distinguish correct paths from incorrect ones \cite{cobbe_2021_ORM,ligthman_PRM,yu-etal-2024-ovm} and are more suited to easy to verify tasks. In the process based verification setting, discriminative verifiers trained as classifiers predict stepwise accuracy scores. These verifier models are trained on carefully curated data, annotated at step-level \cite{ligthman_PRM, uesato_PRM, zhang2025lessonsdevelopingprocessreward}. Given a reasoning step, the models encode the reasoning text and produce the score using a classification head fine-tuned using binary cross-entropy loss. Then the step-level predicted scores are aggregated to get overall correctness of the reasoning and solution \cite{snell_TTS,wu2024scaling}. 


However, manual annotations of stepwise correctness are labor-intensive and hence automated annotation strategies have been proposed for process level annotations \cite{wang-etal-2024-math,luo2024improvemathematicalreasoninglanguage,alphamath} as shown in the data generation phase in Figure \ref{fig:unified_framework}. In the majority of these approaches, a step is considered to be accurate if a valid solution can be sampled from the LLM after k trials through monte-carlo rollouts or other sampling approaches. Hence, the final \textbf{answer accuracy} from rollout determines the value of the current step. However, the subsequent steps after the first error are considered to be incorrect and discarded in all these approaches. Alternatively, AutoCV \cite{autocv} proposes to automate step-level annotations to generate verifier training data by leveraging variations in \textbf{verifier confidence scores} as signal for step-level labels. The approach first trains an ORM based on final answer and uses this ORM iteratively to assign value to the reasoning step at time $t$ based on the variation in confidence scores of ORM after including the step. 
%The process or step-wise labels are obtained based on the confidence variations in output of ORM when the current reasoning step at time $t$ is included. 

While these methods have been successful empirically, it has noted limitations. For instance, \cite{li2025process} observe that PRMs trained this way treat each state independently and do not capture nuances of interaction between steps in a reasoning trajectory, leading to suboptimal reward distribution. To mitigate this issue, \cite{li2025process} propose to redefine the stepwise verification process as a Markov Decision process (MDP). They propose a novel solution for the Q-value ranking problem with a loss function that helps model interdependencies between the steps in the reasoning process.

However, the majority of the above approaches primarily focus on verification for math or code reasoning tasks. However, real-world information needs such as complex Question Answering and fact-checking extend beyond these domains and are commonly called knowledge-intensive tasks. To tackle the lack of verification for these tasks, $Re^2Search++$ \cite{raggym} proposed to train a discriminative PRM using contrastive loss which distinguished preferred actions and solutions from non-preferred ones. The resulting verifier not only checks the intermediate answers but also fine-grained targeted feedback on intermediate actions, such as quality of search queries. In the similar spirit, VersaPRM \cite{zeng2025versaprm} extends to domains beyond math by augmenting the MMLU benchmark with synthetically generated correct and incorrect chains-of-thought (COT) along with step-level annotations. The data is also augmented with counterfactual steps and corresponding correctness annotations to improve the verifier.

In the next section, we discuss limitations of discriminative verifiers and introduce different paradigms of training generative verifiers.


\subsection{Generative verifiers}
\label{sec:generative}
Though the discriminative scoring approach has been shown to be effective on some tasks, it does not utilize the
text-generation capabilities that LLMs are fundamentally designed for. As a result, discriminative RMs miss
out on the inherent strengths of generative LLMs, such as unified instruction tuning ,
chain-of-thought (CoT) reasoning \cite{chainofthought}, and utilizing additional inference-time computation
for better performance \cite{wang2024guiding,brown2024largelanguagemonkeysscaling}. 

  While LLM-as-a-Judge \cite{zhen_llm_judge}, which simply prompts off-the-shelf generative LLMs, also offers the above advantages, it typically underperforms fine-tuned LLMs-based verifiers on reasoning tasks. Hence, more recently training generative ORMs and PRMs has been explored to fill the above mentioned gaps. Based on the training objectives and optimization involved, the generative verifier approaches can be further categorized into: 1) self-verification 2) verifiers trained using classical SFT or 3) verifiers trained using RL as shown in Table \ref{tab:verification} and Figure \ref{fig:categorization_tree}. 

\noindent \textbf{Classical SFT for training generative verifiers:}
One of the first works in training generative verifiers \cite{zhang2024generative}, proposes to employ next token prediction objective to train a LLM jointly on the task of critique generation and verification. The authors generate synthetic rationales which critique the solution candidates (reasoning path and answer) generated. A base LLM acting as verifier in fine-tuned on this using a joint objective to generate critique and final correctness prediction for the candidates. Such verifiers represent solution correctness using the LLM’s probability
distribution over tokens, instead of a separate numerical score. Distillation based classical SFT is also employed in \textbf{self-verification} based approaches \cite{li2025learningreasonfeedbacktesttime,lee2025revise} where models are trained on synthetic verification data from stronger models sometimes augmented with tool based verification data \cite{t1,mekala-etal-2024-toolverifier}. 
  However, the discussed works employing classical SFT to fine-tune verifier do not account for robustness in verifier predictions, casting doubts on reliability. Additionally, studies have observed that lack of robustness in PRMs also leads to reward hacking \cite{ye2025uncertaintyaware}.  To mitigate this issue, Ye et. al. \cite{ye2025uncertaintyaware} propose COT-entropy an \textbf{uncertainty quantification} approach for a generative PRM uses as \textbf{LLM judge} to perform robust process-level verification.

\noindent \textbf{RL-based training of Generative verifiers}: More recently, RL-based training approaches for generative verifiers \cite{hosseini2024vstar,qi2024verifierqenhancingllmtest} has shown potential to have relatively better out-of-distribution performance and reasoning capabilities that are well-aligned to preferences.


V-Star \cite{hosseini2024vstar} improves upon previous self-verification training strategies like StaR \cite{zelikman2022starbootstrappingreasoningreasoning} by sampling correct and incorrect reasoning steps and automatically generating preference data based on their correctness. This is followed by fine-tuning the verifier policy ($\cV_{verifier}$) using Direct preference Optimization (DPO) to increase the likelihood of generating a correct reasoning path and final answer. At inference, the likelihood of solution from the generative verifier is used to rank the candidate solutions. GenRM \cite{mahan2024generativerewardmodels}, adopts a similar approach by collecting correct and incorrect synthetic solution traces to train a generative verifier employing preference optimization.


VerifierQ \cite{qi2024verifierqenhancingllmtest} departs from other RL-based training approaches by employing Q-learning for generative verifiers to enable hybrid scaling. The verifier is trained for Q-value estimation for each step of the solution and can be used to rank multiple solution candidates through parallel estimation. The authors employ Conservative Q-learning which penalizes Q-values exceeding a threshold preventing overestimation issues.

However, above methods still are limited in the sense that when generation is frozen while training the verifier, the verifier is limited by quality of synthetic data from fixed generator and vulnerable to reward hacking and vice versa. 
To prevent reward hacking and reduce generator-verifier gap,
RL-Tango \cite{zha2025rltangoreinforcinggenerator} employs a novel RL-based training framework that co-evolves a generative process-level verifier LLM with the solution generator LLM. The authors employ Group Relative Policy Optimization (GRPO) where the verifier is trained to output step-level predictions for each solution from the generator. The verifier is trained using outcome level correctness as reward and hence does not require process-level manual annotations. The step-level predictions from the verifier are used to improve the generator in the next RL training loop round, improving the quality of solution candidates, which further strengthens the verifier. S2R \cite{ma-etal-2025-s2r} adopts a similar approach but by training the generator LLM to self-verify using outcome level and process-level rewards employing GRPO algorithm. However, generative verifiers still suffer from limitations discussed in the next section.

\subsection{Reasoning based Generative verifiers}

While generative verifier leverage the generative capabilities of LLM for process and outcome verification, they do not necessarily reason over longer trajectories for the tasks that are \textit{``hard to verify"} based on \textbf{asymmetry of verification}. With the advancements in Large Reasoning Models (LRMs), more recently, reasoning based verification models that perform ``thinking" or long-form reasoning for verification of hard to verify tasks have been proposed \cite{thinkJ,khalifa2025processrewardmodelsthink}. 
%Scaling verifiers by through LRMs could help verify complex tasks that are \textit{hard to verify}.

To leverage the benefits of LRMs, ThinkPRM \cite{khalifa2025processrewardmodelsthink}, proposes to train a PRM in generative fashion using a reasoning model as base on synthetic data with automated step-level annotations. The authors demonstrate that through their filtering process they produce high quality synthetic data, which combined with reasoning-based verifier yields superior performance. The resulting verifier is also data-efficient, as it outperforms PRMs trained on \textbf{100 x} more data. 

Similarly, recent approaches also build upon LLM as a judge paradigm and propose to fine-tune LRMs \cite{whitehouse2025j1incentivizingthinkingllmasajudge,thinkJ} to act as judges and rank candidate responses by reasoning for the verification. 


 While the above approaches to train reasoning based verifiers requires enormous data engineering and heuristic design choices, OREO \cite{OREO} produces a verifier naturally as a byproduct of the training framework. OREO \cite{OREO}, proposes an offline RL algorithm that aims to enhance LLM's reasoning capabilities. It accomplishes this by training  a \textit{policy} and \textit{value} function with a LRM as base model jointly by optimizing the ``soft bellman equation" to align as close as possible with the optimal policy, and it's value function. Then the trained value function can be used to guide search in test-time scaling. This is similar in spirit to RL-Tango discussed in Section \ref{sec:generative}.
 
However, above training approaches for verifiers do not focus on robustness and out of domain generalization. Heimdall \cite{heimdall_reasoning_verification}, proposes to fill this gap by generating long-form reasoning chains for the task of verification coupled with RL-based fine-tuning of LRMs for verifiers. It additionally employs a \textit{pessimistic verification} strategy that aims to improve \textbf{robustness} by selecting the most plausible solution with the least uncertainty.



However, all of the discussed approaches allot similar amount of compute to scale the verifier reasoning. However, in the real world deployments not all verification instances are of similar complexity, with some being relatively easy to verify than others. Hence, allotting similar amount of compute for all verification instances could cause issues like overthinking \cite{overthinking} where model produces redundant verification steps even after a correct prediction has been implicitly reached. Hence, approaches like DyVe \cite{zhong2025dyvethinkingfastslow} and FlexiVe \cite{flexive} propose to dynamically adapt compute allocated for verification based on perceived complexity of the verification instance. Inspired by System 1 and 2 thinking \cite{kahneman2011thinking},   alternate between \textbf{fast thinking} which produces immediate token level verification for obviously correct solution steps and \textbf{slow thinking} for solution steps which may require more deliberation, resulting in longer verification reasoning traces based on complexity. DyVe accomplishes this by collecting correct and incorrect reasoning traces for a problem through MCTS rollouts, verifier training data from existing benchmarks like MathShepherd \cite{wang-etal-2024-math}. This is  followed by judgments for each step on whether further elaborate verification is required (System 2). Then a LRM namely  deepseek-ai/DeepSeek-R1-DistillQwen-14B is fine-tuned on this data using cross-entropy loss where it learns to output verification label directly for simpler verification tasks and to perform further reasoning to verify more complex instances. Instead of relying on annotated data on need for further reasoning, FlexiVe \cite{flexive} trains a based model using Group Relative Policy Optimization (GRPO) \cite{deepseek-r1}  on the task of process-level verification. Here, GRPO employs a composite reward, with one reward for to check the correctness of prediction for process verification and another reward which penalizes length of response from the verifier based on accuracy of solution reasoning path. Hence, through this length penalty based reward, the LRM process verifier is incentivized to dynamically adopt fast thinking to verify obviously correct solution steps and slow thinking for hard to verify steps.

While reasoning based generative verifiers help address \textit{hard to verify} tasks, they still suffer from cascading errors due to imprecise step-level annotations. More rigorous verification approaches based on neuro-symbolic methods could help bridge this gap as discussed in the next section.
\subsection{Symbolic Verification}

While much progress has been made in generative PRMs trained on automatically generated data through MCTS rollouts, they still suffer from two fundamental limitations. Firstly, the step-level annotations could be inaccurate or unnatural due to reasoning drift or hallucinations. Secondly, the resulting PRMs still exhibit poor out-of-distribution generalization capabilities. Hence, more robust and formal verification capabilities are required to mitigate inaccuracies. Tasks which can be easily verified through or translated to a form  for formal verification are categorized as \textbf{easy to verify}.

In this section, we discuss training mechanism of verifiers that learn to interact with symbolic systems or LLMs that reason in symbolic format for verification to improve LLM reasoning at inference time. We also cover the class of approaches that generate training data using formal verification tools to train ORMs or PRMs that learn to imitate formal verification.




Deductive PRM \cite{deductive_prm} proposes to perform deductive verification by generating reasoning in rigorous format, namely the natural programs which comprise premise, conditions and statements which can be easily verified. They are generated by prompting stronger models like Gpt-3.5-turbo. The queries with solution steps and verification labels are then employed to \textbf{fine-tune} Vicuna models in a  distillation setup.

In  a similar spirit, SymbCOT \cite{symbCOT} employs strong LLMs to translate COT based reasoning in natural language to symbolic and logic structures (first-order-logic) which is solved step-by-step by another LLM using logical deduction. Then finally, a verification module ensures that the symbolic translation is semantically consistent and also verifies each logic deduction
from solver, to ensure compliance with the principles of formal logic. LMLP \cite{LMLP} follows a similar approach but extends the symbolic programs to facts and logic programs over a knowledge base (KB) supporting automated step-by-step verification of intermediate results for complex Question Answering.

START \cite{li2025startselftaughtreasonertools} departs from above approaches by training a LRM to learn to use symbolic tools adaptively when needed through instruction tuning. The reasoning trajectories in solution candidates from a LRM per query are modified by inserting hints to invoke tools at certain reasoning steps strategically. Then the LRM is further fine-tuned on these trajectories following self-distillation paradigm and learns to invoke symbolic tools for verification adaptively which is leveraged during inference for \textit{sequential} test-time scaling.

While the majority of process-level verifier training and previously discussed symbolic verification approaches rely on distilling step-level annotations from stronger LLMs, EnVISIONS \cite{ENVISIONS} and FOVER \cite{FOVER} \textbf{depart} from these approaches. They rely on neuro-symbolic self-training and symbolic verification tools based data augmentation, respectively.

EnVISIONS \cite{ENVISIONS} proposes an interactive neuro-symbolic training approach that learns to interact with the environment and produce symbolic outputs such as first-order logic form or proofs that can be executed using the environment. The binary feedback from the environment, are converted to soft-rewards and is also employed for self-verification and refinement of symbolic outputs from base LLM without need for human annotation.




FOVER \cite{FOVER} proposes to generate training data with step-level annotations automatically with formal verification tools such as Z3 and Isabelle (formal specification, theorem proving) to train PRMs. The approach first generates a stepwise reasoning process for the task and converts it into a format verifiable by formal verification tools. The formal verification tools provide step-level annotations by verifying and providing error signals, which departs from earlier works that use formal verification tools for entire proofs. The authors demonstrate that process-level verifiers (PRMs) trained on this data exhibits better cross-task generalization (out-of-distribution) by evaluating on logic reasoning benchmarks like ANLI, HANS and MMLU going beyond math and code benchmarks compared to other baseline PRMs. 



==> accuracy_llm_calls.tex <==
\begin{document}
    \begin{tikzpicture}
\begin{axis}[
    xlabel=$x$,
    ylabel=$y$,
    xmin=0, xmax=30,
    ymin=0, ymax=100,
    xtick={10,20,30},
    xticklabels={A,B,X},   % <---
    ytick={0,10,...,100}
            ]
\addplot[smooth,mark=*,blue] plot coordinates {
    (0,10)
    (8,30)
    (16,40)
};
\addlegendentry{Case 1}

\addplot[smooth,color=red,mark=x]
    plot coordinates {
        (4,15)
        (10,25)
        (15,40)
        (18,60)
    };
\addlegendentry{Case 2}
\end{axis}
    \end{tikzpicture}
\end{document}

==> concepts.tex <==
\section{Notions, Terminologies and Concepts}

As scaling models and pre-training data starts to yield diminishing returns in performance, scaling inference time compute has emerged as a new paradigm \cite{snell_TTS}. 
Test-time scaling refers to allotting more compute to LLMs at inference time to explore the space of possible solutions. 
This could entail \textit{parallel scaling} \cite{snell_TTS,lambert2025tulu3pushingfrontiers,brown2024largelanguagemonkeysscaling}, by sampling multiple responses and selecting the best response. More specifically, given a question $q$, related context $c$, a LLM generates multiple candidate solutions $\{1...k\}$ forming the solution space $\cS$, formally  
\[\cS = \mathbb{LLM}(q,c); \ \cS=\{s_1....s_k\} ; \ s^* = \cV(s_1...s_k),\] where $s*$ is one of the correct solutions and $\cV$ is the verification or aggregation approach that derives the final solution from the space of candidate solutions $\cS$. 
Multiple candidate responses could be obtained through repeated sampling by varying the temperature or inducing diversity in exemplars provided as part of prompt \cite{levy-etal-2023-diverse,brown2024largelanguagemonkeysscaling}. The parallel scaling approach has been supported by cognitive science \cite{Stanovich_West_2000, Stanovich_advancing}, which states that complex problems may have more than one correct interpretation and hence more than one valid solution path. 

%Hence, this implies exploring the solution space by sampling multiple solutions increases the chance of arriving at the correct one.
% where the \textbf{``Alternative task construal argument"} implies

Alternatively, \textit{sequential scaling} employs an iterative approach, explicitly conditioning subsequent computations based on intermediate ones. Given a question $q$, sequential scaling breaks this down into sub-questions $\{sq_1...sq_T\}$ where each new sub-question $sq_t = \mathbb(LLM)(sq_{t-1},c_{t})$ is the solution state at time $t$ and is a function of previous state / sub-question, related context ($c_t$) at time $t$.

This is akin to System 2 thinking as described in \cite{kahneman2011thinking} which involves deliberate reasoning for solving a problem and is slower compared to System 1 thinking.

More recently, hybrid scaling approaches have been proposed which interleave parallel and sequential reasoning processes. First, multiple candidate solutions could be explored using parallel scaling, followed by selection and pruning to single or few candidate solutions through sequential scaling. Several search against verifier strategies such as beam search \cite{OREO,snell_TTS}, iterative deepening \cite{iterative_deepening}, tree-of-thoughts \cite{tree_of_thought}, graph-of-thoughts \cite{graph_of_thoughts}, forest-of-thoughts \cite{bi2025forestofthought}, constrained Monte-carlo-tree-search (MCTS) \cite{constrained_MCTS} guided by external verifier or self-verification have been proposed based on this philosophy.

Hence, verifying ($\cV$) the consistency and correctness of LLMs during test-time scaling is crucial for exploration of vast solution space and the selection the best solution. 
Based on whether the verifiers check the final outcome or the intermediate reasoning process to arrive at the outcome, they are categorized into \textbf{outcome} and \textbf{process} verifiers, respectively. 
Hence, based on the verification input, and usage we outline the following approaches:

\paragraph{\textbf{Outcome Verification}}: The model trained to categorize and check if the final solution is correct or incorrect is grouped under this group and commonly referred to as Outcome Reward Models (ORMs) \cite{cobbe_2021_ORM}.

\paragraph{\textbf{Process Verification}}: While outcome reward models (ORMs) are simpler to train they do not consider the step-wise reasoning path that lead to the final answer. This could be problematic, when an incorrect reasoning path from LLM results in the correct answer \cite{creswell2023selectioninference}. Hence, process-based verifiers also termed Process Reward Models (PRMs) mitigate this by validating the reasoning process that leads to the solution in a step-by-step manner. These approaches usually entail training an external verifier on stepwise annotations \cite{uesato_PRM,lightman2024lets,wang-etal-2024-math, autocv}. Alternatively, instead of external verifiers, the LLM could self-critique its solution steps aiding also in self-correction \cite{self_verification_1,lee2025revise,t1}.


==> figures/ablation/sunar_comp_mqa.tex <==

\begin{tikzpicture}
\edef\mylst{"44.58","45.75","54.83"}
\edef\explora{"24.84","0","28.11","32.75","44.28"}

    \begin{axis}[
            ybar=5pt,
            width=4.2cm,
            height=5cm,
            bar width=0.25,
            every axis plot/.append style={fill},
            grid=major,
            xtick={1, 2, 3},
            xticklabels={ PRF, self-ask,\textbf{\name{}}},
            xlabel={},
            ylabel style = {font=\tiny},
        yticklabel style = {font=\boldmath \tiny,xshift=0.05ex},
        xticklabel style ={font=\tiny,yshift=0.5ex},
            ylabel={Task Performance (cover-EM)},
            enlarge x limits=0.25,
            ymin=0,
            ymax=80,
            nodes near coords style={font=\tiny,align=center,text width=2em},
            legend cell align={left},
            legend pos=north west,
            legend columns=-1,
    extra y tick style={grid=major,major grid style={thick,draw=black}}, 
            legend style={/tikz/every even column/.append style={column sep=0.5cm}},
        ]
        \addplot+[
            ybar,
            plotColor1*,
            nodes near coords=\pgfmathsetmacro{\mystring}{{\mylst}[\coordindex]}\textbf{\mystring},
            nodes near coords align={vertical},
            draw=black,
            postaction={
                    pattern=north east lines
                },
        ] plot coordinates {
                (1,44.58)
                (2,45.75)
                (3,54.83)
            };
            
        \draw[color=black, style=densely dashed,line width = 1.5pt] (axis cs:0,65.55) -- (axis cs:5,65.55)  node[pos=0.2, anchor=west, font=\small, yshift=7pt] {Gold};           
    %     \addplot+[
    %         ybar,
    %         plotColor2*,
    %         draw=black,
    %         nodes near coords=\pgfmathsetmacro{\mystring}{{\explora}[\coordindex]}\textbf{\mystring},
    % nodes near coords align={vertical},
    %         postaction={
    %                 pattern=north west lines
    %             },
    %     ] plot coordinates {
    %             (1,24.84)
    %             (2,0)
    %             (3,28.11)
    %             (4,32.75)
    %             (5,44.28 )
    %         };
 

    \end{axis}


    
\end{tikzpicture}


==> figures/time_plot.tex <==
\begin{tikzpicture}

    \begin{axis}[
        ybar=0.2pt,
            width=4cm,
            height=4.2cm,
            bar width=0.25,
            bar shift=0pt,
            every axis plot/.append style={fill},
            grid=major,
            xticklabel style={rotate=10},
            xtick={1, 2},
            xticklabels={\name{}, BoN},
            xlabel={},
            ylabel style = {font= \tiny},
        yticklabel style = {font=\boldmath \tiny, xshift=0.2ex},
        xticklabel style ={font=\small , yshift=0.2ex},
            ylabel={Avg runtime per query },
            enlarge x limits=0.25,
            ymin=0,
            ymax=9200,
            legend style ={font=\small,yshift=0.5ex},
            area legend,
            nodes near coords style={font=\tiny,align=center,text width=2em},
            legend pos=north west,
            legend columns=-1,
            legend style={/tikz/every even column/.append style={column sep=0.2cm}},
        ]
        \addplot+[
            ybar=0.2pt,
            plotColor1*,
            draw=black,
            error bars/.cd,
                y dir=both,
                y explicit,
        ] plot coordinates {
                (1,4970) +- (0,0.38)
            };
            \addplot+[           ybar,
            plotColor2*,
            draw=black,
            postaction={
                    pattern=north east lines
                },
            error bars/.cd,
                y dir=both,
                y explicit,] plot coordinates {           (2,8500) +- (0,0.16)};


 

    \end{axis}
\end{tikzpicture}

==> figures/total_runtime.tex <==
\begin{tikzpicture}

    \begin{axis}[
        ybar=0.2pt,
            width=4cm,
            height=4.2cm,
            bar width=0.25,
            bar shift=0pt,
            every axis plot/.append style={fill},
            grid=major,
            xticklabel style={rotate=10},
            xtick={1, 2},
            xticklabels={\name{}, BoN},
            xlabel={},
            ylabel style = {font= \tiny},
        yticklabel style = {font=\boldmath \tiny, xshift=0.2ex},
        xticklabel style ={font=\small , yshift=0.2ex},
            ylabel={Total runtime per query (in minutes) },
            enlarge x limits=0.25,
            ymin=0,
            ymax=450,
            legend style ={font=\small,yshift=0.5ex},
            area legend,
            nodes near coords style={font=\tiny,align=center,text width=2em},
            legend pos=north west,
            legend columns=-1,
            legend style={/tikz/every even column/.append style={column sep=0.2cm}},
        ]
        \addplot+[
            ybar=0.2pt,
            plotColor1*,
            draw=black,
            error bars/.cd,
                y dir=both,
                y explicit,
        ] plot coordinates {
                (1,206.53)
            };
            \addplot+[           ybar,
            plotColor2*,
            draw=black,
            postaction={
                    pattern=north east lines
                },
            error bars/.cd,
                y dir=both,
                y explicit,] plot coordinates {           (2,349.59) };


 

    \end{axis}
\end{tikzpicture}

==> intro-example.tex <==
\begin{table}[htb!!] % The placement specifier can be [htbp]
\centering
\small
% \scalebox{0.8}{
\begin{tcolorbox}[title=Mitigating \textit{Overthinking} for Numerical FC]
\small
\medskip\noindent \paragraph{\textbf{Claim}:}\texttt{Diaspora remittances “now stand at an all-time high of over KSh400 billion in 2021”.}

[\textbf{Evidence 1}]:  diaspora remittances stand at an all-time-high at over ksh. \textcolor{teal}{400 billion per annum} as of 2021.


[\textbf{Evidence2}]: Diaspora remittances were robust in 2021, with total \textcolor{teal}{remittances in 2021 reaching a record USD $3,718$ million}. of daily users 


 [\textbf{Verdict}]:\textcolor{teal}{\textsf{True}} \\

\textbf{LLM reasoning without \name{}} \\
\textbf{[Reasoning]:} The evidence \textcolor{red}{provides conflicting information} about the exact amount of \textcolor{red}{diaspora remittances} in 2021, and some sources mention figures that \textcolor{red}{are not directly comparable to KSh400 billion.}

\textbf{[Prediction]:} \textcolor{red}{Conflicting} \\


\textbf{LLM reasoning  with \name{}} 

 \textbf{[Reasoning]:}       The evidence supports the claim that diaspora remittances reached an all-time high of over KSh400 billion in 2021. However, \textcolor{teal}{there are minor variations in the wording and units used across different sources.}

 \paragraph{[\textbf{Prediction}]:}\textcolor{teal}{\textsf{True}}
\end{tcolorbox}
% }

\vspace{-1em}
\captionof{figure}{Example numerical claim demonstrating \textit{overthinking} issue and mitigation offered by \name{}}\label{intro:example} 
\end{table}

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

% \color{purple}
% Is our method specific to in-context numerical reasoning, or can it also work for other NLU tasks? What is special about numerical reasoning? Can we say that we design a general method but test it on numerical reasoning tasks because they are more difficult? \color{green} As semantic similarity between train and test set can't be used to select ICEs in case of numerical reasoning. Therefore we propose EXPLORA.\\
% \color{black}
% \color{blue}
% - We are given only the task-specific loss, which is different from generative model error. We do not utilize the logits given by generative models. Bayesian explanation, in-context one iteration GD -- each of these papers, can we say why these theories don't apply to complex QA.

% Complex numerical reasoning tasks such as financial question answering \cite{chen2022finqa} or tabular question answering \cite{tabmwp} require both language understanding as well as reasoning skills.
% Large language models (LLMs) have been shown to exhibit both these skills.
% Language understanding skills help  While 

% \color{gray}

Answering complex questions that require multi-step numerical reasoning \cite{chen2022finqa,tabmwp,aqua_rat,roy2016solving} over structured and unstructured sources is an active research area with applications in finance, law, and healthcare~\cite{wang2023survey}.
% The complexity in such tasks could arise from multiple factors, such as the need to parse heterogeneous sources like tables and text \cite{chen2022finqa} coupled with multi-step numerical reasoning \cite{tabmwp,aqua_rat,roy2016solving} to answer the question. 

Existing supervised approaches for numerical reasoning involve fine-tuning of multiple generative models for generating arithmetic programs or stepwise solution to the original problem \cite{chiang-chen-2019-semantically,amini-etal-2019-mathqa,aqua_rat,roy2016solving,geva-etal-2020-injecting,cobbe_2021_ORM}. 
 
% However, existing approaches require expensive annotations of supervised stepwise rationales along with the solution for fine-tuning multiple generative models \cite{aqua_rat} \cite{} \cite{geva-etal-2020-injecting} lacking a general purpose solution. 

\begin{figure*}[t]
\centering

\includegraphics[width=0.8\textwidth]{figures/explora-cropped.pdf}\\
\caption{Overview of \static{}, proposed exemplar selection approach.}
\label{fig:icl}
% \vspace{-4mm}
\end{figure*}


More recently, the advances in Large Language Models (LLMs) has lead to substantial progress in a wide range of natural language understanding and reasoning tasks \cite{brown2020gpt3}. The emergent capabilities in LLMs\cite{wei2022emergent,gpt3incontext} such as In-Context Learning (ICL) has paved the way to a new class of approaches that employ chain-of-thought reasoning~\cite{complex_cot} \cite{wei2023chainofthought} for solving complex numerical reasoning questions.
Instead of fine-tuning task-specific models, these approaches focus on choosing carefully constructed exemplars with rationales to be used as input to LLMs, commonly termed as prompting.
% A distinct advantage of prompting with demonstration samples vs fine-tuning is  that the LLM is a general-purpose machine that can be used to solve multiple numerical reasoning tasks.
% In this paper, our focus is to propose a general framework that can be employed to solve multiple QA tasks that require numerical reasoning over homogeneous and heterogeneous sources by selecting suitable demonstration samples.

\mpara{The limitations of manual exemplar selection.} 
% It is inherently hard for the LLMs to perform multi-step reasoning using few-shot in-context learning with just the  \texttt{(input, output)} pairs~\cite{rae2022scaling}.
To tackle complex numerical reasoning problems, \textit{chain-of-thought} (COT) prompting was proposed to add hand-crafted natural language rationales (stepwise solutions) to the prompts in addition to input and output resulting in \texttt{(input, rationale, output)}~\cite{wei2023chainofthought}.
% The process of generating stepwise natural language rationales can be seen as decomposing the original problem to simpler problems that can be solved with less effort \cite{wei2023chainofthought} \cite{brown2020gpt3}.

% Interesting, 
% COT rationales for compositional natural language questions involve generating explanations for the final answer. 
% However, such explanations have been found to be unfaithful to the reasoning process of underlying LLM \cite{turpin2023language,ye2022unreliability} for answering compositional questions in complex QA, unlike numerical reasoning questions. 
% In such cases, the decomposition of such question to simpler sub-questions is observed to be more faithful. To induce such decomposition capabilities in LLMs, authors of the work self-ask \cite{self_ask} modify COT prompting and propose to add hand-crafted follow-up questions derived from the original complex questions to the prompt.
However, there are inherent limitations of COT approach for complex and hybrid numerical reasoning tasks. 
The COT involves the manual effort of selecting the best exemplars with appropriate rationales that sufficiently convey the  execution strategy for the task under consideration. The manual selection process is tedious and not scalable across different numerical reasoning tasks. Since the outputs generated by the LLM are highly sensitive to exemplars provided \cite{lu-etal-2022-fantastically,zhao2021calibrate,chang2023data}, it is crucial to select meaningful exemplars that are robust across evaluation samples and improve overall task performance.

\mpara{Limitations of automated exemplar selection approaches}:
To tackle these limitations, several automated exemplar selection approaches have been proposed \cite{ye2023compositional,lu-etal-2022-fantastically,rubin-etal-2022-learning,complex_cot}. These approaches are usually dynamic exemplar selection methods, which select several demonstration examples from the training set for each test example. Several approaches also require annotated data and training of several models for exemplar selection\cite{lu2023dynamic,ye2023compositional}. These approaches entail to heavy computational requirements during inference, especially when there is a large pool of exemplars to select from. While unsupervised approaches like similarity \cite{rubin-etal-2022-learning} or diversity based \cite{ye-etal-2023-complementary} approaches exist for dynamic exemplar selection, they also require projecting the input query and the entire pool of exemplars to a continuous vector space followed by search, increasing computational time during inference. Additionally, the majority of these approaches assume the exemplars chosen to be independent of each other and only consider the interaction between the test sample and the exemplars. They do not account for the interactions between the exemplars themselves.

 As an alternative to dynamic exemplar selection approaches, LENS \cite{li2023finding} proposed to select a static set of task level support exemplars. However, LENS assumes access to language model output logits and involves multiple expensive evaluations of the LLM for scoring the exemplars. LENS also does not model the interactions between exemplars and scores each sample independently. 
% In the example below, using Few-shot-COT results in inaccurate results due to lack of decomposition information in its prompt (hidden due to space reasons).
% \input{intro-example-mouth}

\mpara{\static{} (Static Exemplar Selection Approach):}
In this work, we propose a novel static exemplar selection method \static{}, that selects multiple high value/low loss exemplar subsets. An overview of the working of \static{} is shown in Figure \ref{fig:icl}. The selection of task level exemplar subsets are performed once, and we model the interactions between exemplars through initial sampling of subsets and by directly scoring and selecting subsets. We propose a parameterized scoring function that approximates the loss indicative of task performance using features from a transformer based embedding model. We propose an exploration mechanism as shown in Figure \ref{fig:icl} to estimate the parameters of the scoring function with minimal calls to the LLM and without access to logits from the LLM. Our approach mitigates the expensive processing during inference incurred by traditional dynamic exemplar selection approaches and obviates the need for manual exemplar selection while providing high performance.


\mpara{Contributions.} The core contributions of our work are:
\begin{description}
    \item 
    1) We propose a new robust static exemplar selection approach \static{}, that selects task level exemplars for numerical reasoning based questions.

    \item 
    2) We demonstrate the ability of transferring selected exemplars across models. We show that exemplars selected using smaller models can be used to induce reasoning capabilities in much larger models leading to reduced costs.
     \item 
     3) We demonstrate that \static{} is less resource intensive compared to existing approaches, as it results in minimal calls to the LLMs for exemplar selection.
    \item 
    4) We conduct extensive experiments with different exemplar selection methods to showcase the generalized performance of \static{} across multiple complex and hybrid numerical reasoning based QA tasks.
\end{description}

\color{black}


==> prompts/prompt_decomp.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= DecomP Prompt]
\small
\textbf{Instruction}:\texttt{Solve a question answering task with interleaving retrieval 
Follow the given examples and Given the question and context, use relevant evidence for each subquestion from given list of evidences, answer the subquestion and output final answer for the question using information in the context, answers to subquestions and give final answer strictly preceded by  [Final Answer]:}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138  100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





[Question]: In which country did this Australian who was detained in Guantanamo Bay detention camp
and published Guantanamo: My Journey receive para-military training?


Subquestion 1: (select) [retrieve odqa] Who is the Australian who was detained in Guantanamo Bay detention
camp and published ”Guantanamo: My Journey”?


Answer: {”titles”: [”Guantanamo: My Journey”, ”Bismullah v. Gates”, ”Guantanamo Bay detention
camp”], ”answer”: [”David Hicks”]}


Subquestion 1: (select) [retrieve odqa] In which country did David Hicks receive his para-military training?


Answer: {”titles”: [”John Adams Project”, ”Camp Echo (Guantanamo Bay)”, ”Guantanamo Bay
Museum of Art and History”, ”David Hicks”], ”answer”: [”Afghanistan”]}


Subquestion 3: (select) [multihop titleqa] Titles: [”Guantanamo: My Journey”, ”Bismullah v. Gates”, ”
Guantanamo Bay detention camp”, ”John Adams Project”, ”Camp Echo (Guantanamo Bay)”,
”Guantanamo Bay Museum of Art and History”, ”David Hicks”]. 

Question: In which country
did this Australian who was detained in Guantanamo Bay detention camp and published ``
Guantanamo My Journey" receive para-military training?


[Final Answer]: Afghanistan
\\



[Question]: who is older Jeremy Horn or Renato Sobral ?
Subquestion 1: (select) [retrieve odqa] When was Jeremy Horn born?


Answer: {”titles”: [”Zaza Tkeshelashvili”, ”Jeremy Horn”, ”Jeremy Horn (singer)”, ”Ricardo Arona”], ”
answer”: [”August 25, 1975”]}


Subquestion 2: (select) [retrieve odqa] When was Renato Sobral born?


Answer: {”titles”: [”Brian Warren”, ”Renato Sobral”], ”answer”: [”September 7, 1975”]}


Subquestion 3: (select) [multihop titleqa] Titles: [”Zaza Tkeshelashvili”, ”Jeremy Horn”, ”Jeremy Horn (
singer)”, ”Ricardo Arona”, ”Brian Warren”, ”Renato Sobral”]. Question: who is older Jeremy
Horn or Renato Sobral ?


[Final Answer]: Jeremy Horn
\\

[Question]: What was the 2014 population of the city where Lake Wales Medical Center is located?

Subquestion 1: (select) [retrieve odqa] Lake Wales Medical Center is located in what city?

Answer: {”titles”: [”Baylor College of Medicine”, ”Lake Wales Medical Center”, ”Tufts University
School of Medicine”, ”Hanford Community Medical Center”], ”answer”: [”Polk County,
Florida”]}

Subquestion 2: (select) [retrieve odqa] What was the population of Polk County in 2014?

Answer: {”titles”: [”Banner University Medical Center Tucson”, ”Lake Wales, Florida”], ”answer”:
[”15,140”]}

Subquestion 3: (select) [multihop titleqa] Titles: [”Baylor College of Medicine”, ”Lake Wales Medical Center
”, ”Tufts University School of Medicine”, ”Hanford Community Medical Center”, ”Banner
University Medical Center Tucson”, ”Lake Wales, Florida”]. Question: What was the 2014
population of the city where Lake Wales Medical Center is located?

[Final Answer]: 15,140
\\


[Question]: Nobody Loves You was written by John Lennon and released on what album that was issued
by Apple Records, and was written, recorded, and released during his 18 month separation
from Yoko Ono?

Subquestion 1: (select) [retrieve odqa] What album was issued by Apple Records, and written, recorded, and
released during John Lennon’s 18 month separation from Yoko Ono?

Answer: {”titles”: [”John Lennon/Plastic Ono Band”, ”Milk and Honey (album)”, ”Walls and Bridges”],
”answer”: [”Walls and Bridges”]}

Subquestion 2: (select) [retrieve odqa] Nobody Loves You was written by John Lennon on what album?

Answer: {”titles”: [”John Lennon Museum”, ”Nobody Loves You (When You’re Down and Out)”], ”
answer”: [”Walls and Bridges”]}

Subquestion 3: (select) [multihop titleqa] Titles: [”John Lennon/Plastic Ono Band”, ”Milk and Honey (album)

[Final Answer]: Walls and Bridges
                      [\dots]


\paragraph{\textbf{Input}:} "Follow the above examples, and use the given Evidence: "+\{\}+"  and use the information from the evidence to answer the original question  and give final answer strictly preceded by [Final Answer]: for the   Question: \{\}


\end{tcolorbox}
\captionof{figure}{DeComP prompt \cite{khot2023decomposed}}
\label{prompt:decomp} 
\end{table*}



==> prompts/prompt_meta_reasoner.tex <==
\begin{table}[hbt!]

\begin{tcolorbox}[title= Meta-Reasoner Prompt]
\small
\textbf{Instruction}:\texttt{Follow the given examples and Given the question and context, reasoning path, think step by step extract key segments from given evidence relevant to question and give rationale, by forming your own reasoning path preceded by [Answer]: and output final answer for the question using information from given evidences and give concise precise answer preceded by [Final Answer]:.}



\paragraph{\textbf{Exemplars}}: \{\} \\

Given the above examples and 
\\\textbf{Existing reasoner path}: \{Reasoning path from $\name{}_R$\}, \\
\textbf{the evidence} : \{top-$l$ evidences across sub-questions\} \\ and use the most relevant information for the question from the most relevant evidence from given Evidence: and form your own correct reasoning path to derive the answer thinking step by step preceded by [Answer]: and subsequently give final answer as shown in above examples preceded by [Final Answer]: for \\ \textbf{the Question}: \{Test Question\}

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





\end{tcolorbox}
\captionof{figure}{Meta-reasoner prompt}
\label{fig:meta} 
\end{table}



==> prompts/prompt_react.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= ReAct Prompt]
\small
\textbf{Instruction}:\texttt{Solve a question answering task with interleaving Thought, Action, Observation steps. Thought can reason about the current situation, and Action can be three types: 
(1) Search[entity], which searches the exact entity on Wikipedia and returns the first paragraph if it exists. If not, it will return some similar entities to search.
(2) Lookup[keyword], which returns the next sentence containing keyword in the current passage.
(3) Finish[answer], which returns the answer and finishes the task.:}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





Question: What is the elevation range for the area that the eastern sector of the Colorado orogeny extends into?\\
                Thought 1: I need to search Colorado orogeny, find the area that the eastern sector of the Colorado orogeny extends into, then find the elevation range of the area.\\
                Action 1: Search[Colorado orogeny]\\
                Observation 1: The Colorado orogeny was an episode of mountain building (an orogeny) in Colorado and surrounding areas.\\
                Thought 2: It does not mention the eastern sector. So I need to look up eastern sector.\\
                Action 2: Lookup[eastern sector]\\
                Observation 2: (Result 1 / 1) The eastern sector extends into the High Plains and is called the Central Plains orogeny.\\
                Thought 3: The eastern sector of Colorado orogeny extends into the High Plains. So I need to search High Plains and find its elevation range.\\
                Action 3: Search[High Plains]\\
                Observation 3: High Plains refers to one of two distinct land regions:\\
                Thought 4: I need to instead search High Plains (United States).\\
                Action 4: Search[High Plains (United States)]\\
                Observation 4: The High Plains are a subregion of the Great Plains. From east to west, the High Plains rise in elevation from around 1,800 to 7,000 ft (550 to 2,130 m).[3]\\
                Thought 5: High Plains rise in elevation from around 1,800 to 7,000 ft, so the answer is 1,800 to 7,000 ft.\\
                Action 5: Finish[1,800 to 7,000 ft]

                
                [Final Answer]: 1,800 to 7,000 ft \\
                Question: Musician and satirist Allie Goertz wrote a song about the \"The Simpsons\" character Milhouse, who Matt Groening named after who?\\
                Thought 1: The question simplifies to \"The Simpsons\" character Milhouse is named after who. I only need to search Milhouse and find who it is named after.\\
                Action 1: Search[Milhouse]\\
                Observation 1: Milhouse Mussolini Van Houten is a recurring character in the Fox animated television series The Simpsons voiced by Pamela Hayden and created by Matt Groening.\\
                Thought 2: The paragraph does not tell who Milhouse is named after, maybe I can look up \"named after\".\\
                Action 2: Lookup[named after]\\Observation 2: (Result 1 / 1) Milhouse was named after U.S. president Richard Nixon, whose middle name was Milhous. \\
                Thought 3: Milhouse was named after U.S. president Richard Nixon, so the answer is Richard Nixon.\\
                Action 3: Finish[Richard Nixon]\\Question: Which documentary is about Finnish rock groups, Adam Clayton Powell or The Saimaa Gesture?\\
                Thought 1: I need to search Adam Clayton Powell and The Saimaa Gesture, and find which documentary is about Finnish rock groups.\\
                Action 1: Search[Adam Clayton Powell]\\
                Observation 1: Could not find [Adam Clayton Powell]. Similar: ['Adam Clayton Powell III', 'Seventh Avenue (Manhattan)', 'Adam Clayton Powell Jr. State Office Building', 'Isabel Washington Powell', 'Adam Powell', 'Adam Clayton Powell (film)', 'Giancarlo Esposito'].\\
                Thought 2: To find the documentary, I can search Adam Clayton Powell (film).\\
                Action 2: Search[Adam Clayton Powell (film)]\\
                Observation 2: Adam Clayton Powell is a 1989 American documentary film directed by Richard Kilberg.\\
                The film is about the rise and fall of influential African-American politician Adam Clayton Powell Jr.[3][4] It was later aired as part of the PBS series The American Experience.\\
                Thought 3: Adam Clayton Powell (film) is a documentary about an African-American politician, not Finnish rock groups. So the documentary about Finnish rock groups must instead be The Saimaa Gesture.\\
                Action 3: Finish[The Saimaa Gesture]

                
                [Final Answer]: The Saimaa Gesture \\

  
[\dots]

\paragraph{\textbf{Input}:} "Follow the above examples, and use the given Evidence: "+\{\}+" \\ and use the information from the evidence to answer the original question  and give final answer strictly preceded by [Final Answer]: for the   Question: \{\}
\end{tcolorbox}
\captionof{figure}{ReAct prompt \cite{khot2023decomposed}}
\label{prompt:react} 
\end{table*}



==> prompts/prompt_searchain.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= SearChain Prompt]
\small
\textbf{Instruction}:\texttt{Solve a question answering task with interleaving Thought, Action, Observation steps. Thought can reason about the current situation, and Action can be three types: 
(1) Search[entity], which searches the exact entity on Wikipedia and returns the first paragraph if it exists. If not, it will return some similar entities to search. \\
(2) Lookup[keyword], which returns the next sentence containing keyword in the current passage. \\
(3) Finish[answer], which returns the answer and finishes the task.}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





Question: When does monsoon season end in the state the area code 575 is located? \\
Are follow up questions needed here: Yes. \\
Follow up: Which state is the area code 575 located in?\\
Intermediate Answer: The area code 575 is located in New Mexico. \\
Follow up: When does monsoon season end in New Mexico? \\
Intermediate Answer: Monsoon season in New Mexico typically ends in mid-September. 

[Final Answer]: mid-September. 
\\


Construct a global reasoning chain for this complex [Question] : " \{\} " You should generate a query to the search engine based on
        what you already know at each step of the reasoning chain, starting with [Query]. \\
                        If you know the answer for [Query], generate it starting with [Answer]. \\
                        You can try to generate the final answer for the [Question] by referring to the [Query]-[Answer] pairs, starting with [Final
                        Answer].\\
                        If you don't know the answer, generate a query to search engine based on what you already know and do not know, starting with
                        [Unsolved Query]. \\
                        For example:
                        [Question]: "Where do greyhound buses that are in the birthplace of Spirit If...'s performer leave from? "

                        
                        [Query 1]: Who is the performer of Spirit If... ? \\
                        If you don't know the answer: 

                        
                        [Unsolved Query]: Who is the performer of Spirit If... ? \\
                        If you know the answer:
                        [Answer 1]: The performer of Spirit If... is Kevin Drew.
                        [Query 2]: Where was Kevin Drew born? \\
                        If you don't know the answer:
                        [Unsolved Query]: Where was Kevin Drew born? \\
                        If you know the answer:
                        [Answer 2]: Toronto. 
                        
                        [Query 3]: Where do greyhound buses in Toronto leave from? \\
                        If you don't know the answer:
                        [Unsolved Query]: Where do greyhound buses in Toronto leave from? \\
                        If you know the answer:
                        [Answer 3]: Toronto Coach Terminal. 
                        
                        [Final Content]: The performer of Spirit If... is Kevin Drew [1]. Kevin Drew was born in Toronto [2]. Greyhound buses in
                        Toronto leave from Toronto
                        Coach Terminal [3]. So the final answer is Toronto Coach Terminal. 
                        
                        [Final Answer]: Toronto Coach Terminal 

                        
                        [Question]:"Which magazine was started first Arthur’s Magazine or First for Women?" 

                        
                        [Query 1]: When was Arthur’s Magazine started? 

                        
                        [Answer 1]: 1844. 

                        
                        [Query 2]: When was First for Women started?
                        [Answer 2]: 1989 

                        
                        [Final Content]: Arthur’s Magazine started in 1844 [1]. First for Women started in 1989 [2]. So Arthur’s Magazine was started
                        first. So the answer is Arthur’s Magazi 
                        

                        
                        [Final Answer]: Arthur’s Magazi.
                      [\dots]




\end{tcolorbox}
\captionof{figure}{Searchain prompt used for complex QA \cite{xu2024searchinthechaininteractivelyenhancinglarge}}
\label{prompt:searchain} 
\end{table*}



==> prompts/self_ask_prompt.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= \self{} 2WikiMultiHopQA Prompt]
\small
\textbf{Instruction}:\texttt{Follow the given examples and Given the question determine if followup questions are needed and decompose the original question.}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





Question: Who lived longer, Theodor Haecker or Harry Vaughan Watkins? \\
                Are follow up questions needed here: Yes.\\
Follow up: How old was Theodor Haecker when he died?\\
Intermediate Answer: Theodor Haecker was 65 years old when he died.\\
Follow up: How old was Harry Vaughan Watkins when he died?\\
Intermediate Answer: Harry Vaughan Watkins was 69 years old when he died.

[Final Answer]: Harry Vaughan Watkins.
\\
Question: Why did the founder of Versus die? \\
Are follow up questions needed here: Yes.\\
Follow up: Who founded Versus?\\
Intermediate Answer: Gianni Versace.\\
Follow up: Why did Gianni Versace die?\\
Intermediate Answer: Gianni Versace was shot and killed on the steps of his Miami Beach mansion on July 15, 1997.
[Final Answer]: Shot.
\\
Question: Who is the grandchild of Dambar Shah? \\
Are follow up questions needed here: Yes. \\
Follow up: Who is the child of Dambar Shah? \\
Intermediate Answer: Dambar Shah (? - 1645) was the king of the Gorkha Kingdom. He was the father of Krishna Shah. \\
Follow up: Who is the child of Krishna Shah? \\
Intermediate Answer: Krishna Shah (? - 1661) was the king of the Gorkha Kingdom. He was the father of Rudra Shah. 
[Final Answer]: Rudra Shah.
\\
Question: Are both director of film FAQ: Frequently Asked Questions and director of film The Big Money from the same
country? \\
Are follow up questions needed here: Yes. \\
Follow up: Who directed the film FAQ: Frequently Asked Questions?\\
Intermediate Answer: Carlos Atanes.\\
Follow up: Who directed the film The Big Money?
Intermediate Answer: John Paddy Carstairs.
Follow up: What is the nationality of Carlos Atanes?
Intermediate Answer: Carlos Atanes is Spanish.
Follow up: What is the nationality of John Paddy Carstairs?\\
Intermediate Answer: John Paddy Carstairs is British.
[Final Answer]: No.
\\
Question: Who was the maternal grandfather of George Washington? \\
Are follow up questions needed here: Yes.
Follow up: Who was the mother of George Washington?\\
Intermediate answer: The mother of George Washington was Mary Ball Washington. \\
Follow up: Who was the father of Mary Ball Washington? \\
Intermediate answer: The father of Mary Ball Washington was Joseph Ball.
[Final Answer]: Joseph Ball 
\\


\paragraph{\textbf{Input}}: Based on above examples, given the Question: {} determine, Are followup questions needed here ?




\end{tcolorbox}
\captionof{figure}{Example of In-context learning for 2WikiMultiHopQA through \self{} based prompting of LLMs }
\label{prompt:wqa} 
\end{table*}



==> prompts/self_ask_prompt_mqa.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= \self{} MusiqueQA Prompt]
\small
\textbf{Instruction}:\texttt{Follow the given examples and Given the question determine if followup questions are needed and decompose the original question.}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





Question: When does monsoon season end in the state the area code 575 is located? \\
Are follow up questions needed here: Yes. \\
Follow up: Which state is the area code 575 located in?\\
Intermediate Answer: The area code 575 is located in New Mexico. \\
Follow up: When does monsoon season end in New Mexico? \\
Intermediate Answer: Monsoon season in New Mexico typically ends in mid-September. 

[Final Answer]: mid-September. 
\\


Question: What is the current official currency in the country where Ineabelle Diaz is a citizen? \\
Are follow up questions needed here: Yes. \\
Follow up: Which country is Ineabelle Diaz a citizen of? \\
Intermediate Answer: Ineabelle Diaz is from Peurto Rico, which is in the United States of America. \\
Follow up: What is the current official currency in the United States of America? \\
Intermediate Answer: The current official currency in the United States is the United States dollar.
[Final Answer]: United States dollar.
\\

Question: Where was the person who founded the American Institute of Public Opinion in 1935 born?
Are follow up questions needed here: Yes.
Follow up: Who founded the American Institute of Public Opinion in 1935?
Intermediate Answer: George Gallup.
Follow up: Where was George Gallup born?
Intermediate Answer: George Gallup was born in Jefferson, Iowa.

[Final Answer]: Jefferson.
\\


Question: What is the sports team the person played for who scored the first touchdown in Superbowl 1?  \\
Are follow up questions needed here: Yes. \\
Follow up: Which player scored the first touchdown in Superbowl 1? \\
Intermediate Answer: Max McGee. \\
Follow up: Which sports team did Max McGee play for? \\
Intermediate Answer: Max McGee played for the Green Bay Packers.

[Final Answer]: Green Bay Packers.
\\

Question: The birth country of Jayantha Ketagoda left the British Empire when? \\
Are follow up questions needed here: Yes. \\
Follow up: What is the birth country of Jayantha Ketagoda? \\
Intermediate Answer: Sri Lanka. \\
Follow up: When did Sri Lanka leave the British Empire? \\
Intermediate Answer: Sri Lanka left the British Empire on February 4, 1948. 

[Final Answer]: February 4, 1948 \\
                      
\paragraph{\textbf{Input}}: Based on above examples, given the Question: {} determine, Are followup questions needed here ?




\end{tcolorbox}
\captionof{figure}{Example of In-context learning for MusiqueQA (MQA) through \self{} based prompting of LLMs}
\label{prompt:mqa} 
\end{table*}



==> tables/reward_model.tex <==
\begin{table*}[htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Per Class F1}} & \multicolumn{2}{c}{\textbf{Overall F1 Score}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-6}
& \textbf{T-F1} & \textbf{F-F1} & \textbf{C-F1} & \textbf{Macro} & \textbf{Weighted} \\
\midrule
\textbf{Llama-3.1 8B} \\
% \multicolumn{6}{l}{\textbf{Majority voting}} \\
% \midrule

Top 1 Decoding & 33.5  & 66.4 & 34.7   & 44.8  & 52.5 \\

Self-Consistency \cite{self_consistency} & 
34.9 & 
68.6 & 
35.1 & 
46.2 & 
54.2 \\

Best of N (\name{}) & 
\textbf{44.2} (\textcolor{darkgreen}{+31.9\%}) & 
\textbf{75.3} (\textcolor{darkgreen}{+13.4\%}) & 
\textbf{40.3} (\textcolor{darkgreen}{+16.1\%}) & 
\textbf{53.2} (\textcolor{darkgreen}{+18.8\%}) & 
\textbf{61.0} (\textcolor{darkgreen}{+16.2\%}) \\

Theoretical upper bound & 63.9  & 85.1 & 69.6   & 72.9  & 77.4 \\
\midrule
\textbf{Gpt-4o-mini} \\
Top 1 decoding & 40.68 & 63.14 & 37.99 &47.27 & 52.84 \\
Self-Consistency \cite{self_consistency} & 29.70 & 63.20 & 42.33 & 45.07 & 51.83 \\
Best of N (\name{}) & &   \\
Theoretical upper bound & 45.34 & 85.37 & 67.19 & 65.97 & 73.41 \\

\bottomrule
\end{tabular}}

\captionsetup{font=small}
\caption{Reasoning performance of the models. Here the number of samples for majority voting and best of N sampling is set to 10. The generator model is llama-3.1-Instruct-8b, and the reward model is fine-tuned llama-3.2-3b. The gains method is computed w.r.t the \textit{top 1 Decoding} baseline.}
\label{tab:rm_performance_table}
\end{table*}

==> tables/taxonomy.tex <==
\begin{figure*}[t!]
    \centering
    \tikzstyle{my-box}=[
        rectangle,
        rounded corners,
        minimum height=0.1em,
        minimum width=0.1em,
        inner sep=2pt,
        align=left,
        fill opacity=.5,
        text opacity=1,
    ]
    \tikzstyle{leaf}=[my-box]

    \resizebox{0.48\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\fontsize{6}{6}\selectfont,
                rectangle,
                rounded corners,
                align=left,
                minimum width=0.1em,
                edge+={darkgray, line width=0.8pt},
                s sep=2pt,
                inner xsep=2pt,
                inner ysep=2pt,
                draw=hidden-draw,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=4.8em,font=\fontsize{4.5}{5.5}\selectfont,}{},
            where level=2{text width=6em,font=\fontsize{4}{4.5}\selectfont,}{},
            where level=3{text width=6.5em,font=\fontsize{4.2}{4.5}\selectfont,}{},
            where level=4{text width=7em,font=\fontsize{4.5}{4.5}\selectfont,}{},
            [
                Test-Time Verifiers, draw=black, fill=gray!10, thick, text=black, ver
                [
                    Verification Scope (~\S\ref{sec:scope}),
                    color=blue!80, fill=blue!15, thick, text=black
                    [
                        Outcome-Level,
                        color=blue!80, fill=blue!15, thick, text=black
                        [
                            Naive ORM, color=black!80, fill=gray!10
                        ]
                        [
                            OVM, color=black!80, fill=gray!10
                        ]
                        [
                            Heuristic, color=black!80, fill=gray!10
                        ]
                        [
                            Functional, color=black!80, fill=gray!10
                        ]
                        [
                            Bandit, color=black!80, fill=gray!10
                        ]
                        [
                            Generative Verifier, color=black!80, fill=gray!10
                        ]
                        [
                            Self-Reflection, color=black!80, fill=gray!10
                        ]
                        [
                            Discriminator (ToT), color=black!80, fill=gray!10
                        ]
                        [
                            Unit Test, color=black!80, fill=gray!10
                        ]
                        [
                            XoT, color=black!80, fill=gray!10
                        ]
                        [
                            WoT, color=black!80, fill=gray!10
                        ]
                        [
                            Multi-Agent, color=black!80, fill=gray!10
                        ]
                    ]
                    [
                        Process-Level,
                        color=blue!80, fill=blue!15, thick, text=black
                        [
                            Naive PRM, color=black!80, fill=gray!10
                        ]
                        [
                            State Verifier, color=black!80, fill=gray!10
                        ]
                        [
                            Deductive PRM, color=black!80, fill=gray!10
                        ]
                        [
                            Self-Evaluation, color=black!80, fill=gray!10
                        ]
                        [
                            Lego-Prover, color=black!80, fill=gray!10
                        ]
                        [
                            Tool Verifier, color=black!80, fill=gray!10
                        ]
                        [
                            V-STaR, color=black!80, fill=gray!10
                        ]
                    ]
                ]
                [
                    Verifier Architecture (~\S\ref{sec:arch}),
                    color=red!80, fill=red!15, thick, text=black
                    [
                        Discriminative,
                        color=red!80, fill=red!15
                        [
                            Naive ORM
                        ]
                        [
                            Naive PRM
                        ]
                        [
                            Discriminator
                        ]
                        [
                            State Verifier
                        ]
                        [
                            V-STaR
                        ]
                    ]
                    [
                        Generative,
                        color=red!80, fill=red!15
                        [
                            Generative Verifier
                        ]
                    ]
                    [
                        Self-Reflective,
                        color=red!80, fill=red!15
                        [
                            Self-Evaluation
                        ]
                        [
                            Self-Reflection Feedback
                        ]
                    ]
                    [
                        Heuristic / Rule-based,
                        color=red!80, fill=red!15
                        [
                            Heuristic
                        ]
                        [
                            Functional
                        ]
                        [
                            Deductive PRM
                        ]
                    ]
                    [
                        Tool-based,
                        color=red!80, fill=red!15
                        [
                            Unit Test
                        ]
                        [
                            Tool Verifier
                        ]
                        [
                            Lego-Prover
                        ]
                        [
                            XoT
                        ]
                    ]
                    [
                        Bandit / RL,
                        color=red!80, fill=red!15
                        [
                            OVM
                        ]
                        [
                            Bandit
                        ]
                    ]
                    [
                        Multi-Agent,
                        color=red!80, fill=red!15
                        [
                            WoT
                        ]
                        [
                            Multi-Agent
                        ]
                    ]
                ]
                [
                    Interaction Type (~\S\ref{sec:interaction}),
                    color=green!80, fill=green!20, thick, text=black
                    [
                        Passive,
                        color=green!80, fill=green!20
                        [
                            Naive ORM
                        ]
                        [
                            Heuristic
                        ]
                        [
                            Functional
                        ]
                        [
                            Naive PRM
                        ]
                        [
                            State Verifier
                        ]
                        [
                            Deductive PRM
                        ]
                        [
                            Unit Test
                        ]
                        [
                            Tool Verifier
                        ]
                        [
                            V-STaR
                        ]
                        [
                            Multi-Agent
                        ]
                        [
                            Discriminator
                        ]
                    ]
                    [
                        Active,
                        color=green!80, fill=green!20
                        [
                            OVM
                        ]
                        [
                            Bandit
                        ]
                        [
                            Generative Verifier
                        ]
                        [
                            Self-Reflection Feedback
                        ]
                        [
                            XoT
                        ]
                        [
                            WoT
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{Taxonomy of test-time verification methods for LLMs, based on verification scope, architecture, and interaction type.}
    \label{fig:verifier-taxonomy}
\end{figure*}
